Fresco++: Frequency-Guided and Canonical-Consistent Optimization for Fine-Grained Head Avatar Modeling

We propose Fresco++, a unified optimization framework for fine-grained and view-consistent head avatar reconstruction. Head avatar optimization is typically driven by per-view image supervision, which can lead to premature fitting of unstable high-frequency details and inconsistent local appearance across viewpoints. Fresco++ addresses these challenges by regulating both the progression of visual detail and the formation of cross-view supervision during optimization. For frequency-aware optimization, a progressive curriculum first stabilizes low-frequency structures and then introduces high-frequency constraints to recover fine facial and hair details without amplifying spurious responses at early stages. For cross-view optimization, we introduce Canonical Group Consensus, which associates local observations through shared canonical surface regions and establishes correspondence across different viewpoints. Geometric and visibility-aware screening removes unreliable observations, while the remaining multi-view evidence is aggregated in feature space to form a consensus target for supervising the current rendering. This design enforces local consistency without relying on a specific image-space parameterization and avoids additional rendering of the auxiliary view. Together, the frequency curriculum and canonical consensus provide stable optimization from coarse structures to fine details while maintaining coherent appearance across viewpoints. Extensive experiments on NeRSemble demonstrate improved reconstruction quality and cross-view consistency, while evaluations across diverse avatar representations further confirm the generality and transferability of Fresco++.

==> references_thebibliography.tex <==
\begin{thebibliography}{99}

\bibitem{waggoner2009my}
Z. Waggoner, \textit{My avatar, my self: Identity in video role-playing games}. McFarland, 2009.

\bibitem{he2020collabovr}
Z. He, R. Du, and K. Perlin, ``Collabovr: A reconfigurable framework for creative collaboration in virtual reality,'' in \textit{2020 IEEE International Symposium on Mixed and Augmented Reality (ISMAR)}, pp. 542--554, 2020.

\bibitem{lombardi2018deep}
S. Lombardi, J. Saragih, T. Simon, and Y. Sheikh, ``Deep appearance models for face rendering,'' \textit{ACM Transactions on Graphics (ToG)}, vol. 37, no. 4, pp. 1--13, 2018.

\bibitem{orts2016holoportation}
S. Orts-Escolano, C. Rhemann, S. Fanello, W. Chang, A. Kowdle, Y. Degtyarev, D. Kim, P. L. Davidson, S. Khamis, M. Dou, et al., ``Holoportation: Virtual 3d teleportation in real-time,'' in \textit{Proceedings of the 29th annual symposium on user interface software and technology}, pp. 741--754, 2016.

\bibitem{barron2021mip}
J. T. Barron, B. Mildenhall, M. Tancik, P. Hedman, R. Martin-Brualla, and P. P. Srinivasan, ``Mip-nerf: A multiscale representation for anti-aliasing neural radiance fields,'' in \textit{Proceedings of the IEEE/CVF international conference on computer vision}, pp. 5855--5864, 2021.

\bibitem{chen2022tensorf}
A. Chen, Z. Xu, A. Geiger, J. Yu, and H. Su, ``Tensorf: Tensorial radiance fields,'' in \textit{European conference on computer vision}, pp. 333--350, 2022.

\bibitem{mildenhall2021nerf}
B. Mildenhall, P. P. Srinivasan, M. Tancik, J. T. Barron, R. Ramamoorthi, and R. Ng, ``Nerf: Representing scenes as neural radiance fields for view synthesis,'' \textit{Communications of the ACM}, vol. 65, no. 1, pp. 99--106, 2021.

\bibitem{muller2022instant}
T. M{\"u}ller, A. Evans, C. Schied, and A. Keller, ``Instant neural graphics primitives with a multiresolution hash encoding,'' \textit{ACM transactions on graphics (TOG)}, vol. 41, no. 4, pp. 1--15, 2022.

\bibitem{hong2022headnerf}
Y. Hong, B. Peng, H. Xiao, L. Liu, and J. Zhang, ``Headnerf: A real-time nerf-based parametric head model,'' in \textit{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pp. 20374--20384, 2022.

\bibitem{wang2023neural}
C. Wang, D. Kang, Y. Cao, L. Bao, Y. Shan, and S. Zhang, ``Neural point-based volumetric avatar: Surface-guided neural points for efficient and photorealistic volumetric head avatar,'' in \textit{SIGGRAPH Asia 2023 Conference Papers}, pp. 1--12, 2023.

\bibitem{xu2023avatarmav}
Y. Xu, L. Wang, X. Zhao, H. Zhang, and Y. Liu, ``Avatarmav: Fast 3d head avatar reconstruction using motion-aware neural voxels,'' in \textit{ACM SIGGRAPH 2023 Conference Proceedings}, pp. 1--10, 2023.

\bibitem{wang2021neus}
P. Wang, L. Liu, Y. Liu, C. Theobalt, T. Komura, and W. Wang, ``Neus: Learning neural implicit surfaces by volume rendering for multi-view reconstruction,'' \textit{arXiv preprint arXiv:2106.10689}, 2021.

\bibitem{yariv2021volume}
L. Yariv, J. Gu, Y. Kasten, and Y. Lipman, ``Volume rendering of neural implicit surfaces,'' \textit{Advances in neural information processing systems}, vol. 34, pp. 4805--4815, 2021.

\bibitem{dhamo2024headgas}
H. Dhamo, Y. Nie, A. Moreau, J. Song, R. Shaw, Y. Zhou, and E. P{\'e}rez-Pellitero, ``Headgas: Real-time animatable head avatars via 3d gaussian splatting,'' in \textit{European Conference on Computer Vision}, pp. 459--476, 2024.

\bibitem{qian2024gaussianavatars}
S. Qian, T. Kirschstein, L. Schoneveld, D. Davoli, S. Giebenhain, and M. Nie{\ss}ner, ``Gaussianavatars: Photorealistic head avatars with rigged 3d gaussians,'' in \textit{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pp. 20299--20309, 2024.

\bibitem{wang2025gaussianhead}
J. Wang, J. Xie, X. Li, F. Xu, C. Pun, and H. Gao, ``Gaussianhead: High-fidelity head avatars with learnable gaussian derivation,'' \textit{IEEE Transactions on Visualization and Computer Graphics}, 2025.

\bibitem{xiang2024flashavatar}
J. Xiang, X. Gao, Y. Guo, and J. Zhang, ``Flashavatar: High-fidelity head avatar with efficient gaussian embedding,'' in \textit{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pp. 1802--1812, 2024.

\bibitem{gafni2021dynamic}
G. Gafni, J. Thies, M. Zollhofer, and M. Nie{\ss}ner, ``Dynamic neural radiance fields for monocular 4d facial avatar reconstruction,'' in \textit{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pp. 8649--8658, 2021.

\bibitem{zheng2022avatar}
Y. Zheng, V. F. Abrevaya, M. C. B{\"u}hler, X. Chen, M. J. Black, and O. Hilliges, ``Im avatar: Implicit morphable head avatars from videos,'' in \textit{Proceedings of the IEEE/CVF conference on computer vision and pattern recognition}, pp. 13545--13555, 2022.

\bibitem{li2017learning}
T. Li, T. Bolkart, M. J. Black, H. Li, and J. Romero, ``Learning a model of facial shape and expression from 4D scans,'' \textit{ACM Trans. Graph.}, vol. 36, no. 6, pp. 194--1, 2017.

\bibitem{grassal2022neural}
P. Grassal, M. Prinzler, T. Leistner, C. Rother, M. Nie{\ss}ner, and J. Thies, ``Neural head avatars from monocular rgb videos,'' in \textit{Proceedings of the IEEE/CVF conference on computer vision and pattern recognition}, pp. 18653--18664, 2022.

\bibitem{zheng2023pointavatar}
Y. Zheng, W. Yifan, G. Wetzstein, M. J. Black, and O. Hilliges, ``Pointavatar: Deformable point-based head avatars from videos,'' in \textit{Proceedings of the IEEE/CVF conference on computer vision and pattern recognition}, pp. 21057--21067, 2023.

\bibitem{guedon2024sugar}
A. Gu{\'e}don and V. Lepetit, ``Sugar: Surface-aligned gaussian splatting for efficient 3d mesh reconstruction and high-quality mesh rendering,'' in \textit{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pp. 5354--5363, 2024.

\bibitem{wang2025mega}
C. Wang, D. Kang, H. Sun, S. Qian, Z. Wang, L. Bao, and S. Zhang, ``Mega: Hybrid mesh-gaussian head avatar for high-fidelity rendering and head editing,'' in \textit{Proceedings of the Computer Vision and Pattern Recognition Conference}, pp. 26274--26284, 2025.

\bibitem{xu2024gaussian}
Y. Xu, B. Chen, Z. Li, H. Zhang, L. Wang, Z. Zheng, and Y. Liu, ``Gaussian head avatar: Ultra high-fidelity head avatar via dynamic gaussians,'' in \textit{Proceedings of the IEEE/CVF conference on computer vision and pattern recognition}, pp. 1931--1941, 2024.

\bibitem{cai2024hybrid}
H. Cai, Y. Xiao, X. Wang, J. Li, Y. Guo, Y. Fan, S. Gao, and J. Zhang, ``Hybrid Explicit Representation for Ultra-Realistic Head Avatars,'' \textit{arXiv preprint arXiv:2403.11453}, 2024.

\bibitem{zhang2025eavatar}
S. Zhang, C. Chen, Y. Wang, Q. Ke, and Y. Li, ``EAvatar: Expression-Aware Head Avatar Reconstruction with Generative Geometry Priors,'' \textit{arXiv preprint arXiv:2508.13537}, 2025.

\bibitem{lin2021barf}
C. Lin, W. Ma, A. Torralba, and S. Lucey, ``Barf: Bundle-adjusting neural radiance fields,'' in \textit{Proceedings of the IEEE/CVF international conference on computer vision}, pp. 5741--5751, 2021.

\bibitem{yang2023freenerf}
J. Yang, M. Pavone, and Y. Wang, ``Freenerf: Improving few-shot neural rendering with free frequency regularization,'' in \textit{Proceedings of the IEEE/CVF conference on computer vision and pattern recognition}, pp. 8254--8263, 2023.

\bibitem{zhang2024fregs}
J. Zhang, F. Zhan, M. Xu, S. Lu, and E. Xing, ``Fregs: 3d gaussian splatting with progressive frequency regularization,'' in \textit{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pp. 21424--21433, 2024.

\bibitem{thies2019deferred}
J. Thies, M. Zollh{\"o}fer, and M. Nie{\ss}ner, ``Deferred neural rendering: Image synthesis using neural textures,'' \textit{Acm Transactions on Graphics (TOG)}, vol. 38, no. 4, pp. 1--12, 2019.

\bibitem{kirschstein2023nersemble}
T. Kirschstein, S. Qian, S. Giebenhain, T. Walter, and M. Nie{\ss}ner, ``Nersemble: Multi-view radiance field reconstruction of human heads,'' \textit{ACM Transactions on Graphics (TOG)}, vol. 42, no. 4, pp. 1--14, 2023.

\bibitem{lee2020maskgan}
C. Lee, Z. Liu, L. Wu, and P. Luo, ``Maskgan: Towards diverse and interactive facial image manipulation,'' in \textit{Proceedings of the IEEE/CVF conference on computer vision and pattern recognition}, pp. 5549--5558, 2020.

\bibitem{over2021processing}
J. R. Over, A. C. Ritchie, C. J. Kranenburg, J. A. Brown, D. D. Buscombe, T. Noble, C. R. Sherwood, J. A. Warrick, and P. A. Wernette, ``Processing coastal imagery with Agisoft Metashape Professional Edition, version 1.6—Structure from motion workflow documentation,'' US Geological Survey, 2021.

\bibitem{park2021nerfies}
K. Park, U. Sinha, J. T. Barron, S. Bouaziz, D. B. Goldman, S. M. Seitz, and R. Martin-Brualla, ``Nerfies: Deformable neural radiance fields,'' in \textit{Proceedings of the IEEE/CVF international conference on computer vision}, pp. 5865--5874, 2021.

\bibitem{kerbl20233d}
B. Kerbl, G. Kopanas, T. Leimk{\"u}hler, and G. Drettakis, ``3D Gaussian splatting for real-time radiance field rendering,'' \textit{ACM Trans. Graph.}, vol. 42, no. 4, pp. 139--1, 2023.

\bibitem{liao2025hhavatar}
Z. Liao, Y. Xu, Z. Li, Q. Li, B. Zhou, R. Bai, D. Xu, H. Zhang, and Y. Liu, ``HHAvatar: Gaussian head avatar with dynamic hairs,'' \textit{IEEE Transactions on Pattern Analysis and Machine Intelligence}, 2025.

\bibitem{xu2025gphm}
Y. Xu, Z. Su, Q. Wu, and Y. Liu, ``Gphm: Gaussian parametric head model for monocular head avatar reconstruction,'' \textit{IEEE Transactions on Pattern Analysis and Machine Intelligence}, 2025.

\bibitem{wang20253d}
Y. Wang, X. Wang, R. Yi, Y. Fan, J. Hu, J. Zhu, and L. Ma, ``3D Gaussian Head Avatars with Expressive Dynamic Appearances by Compact Tensorial Representations,'' in \textit{Proceedings of the Computer Vision and Pattern Recognition Conference}, pp. 21117--21126, 2025.

\bibitem{qin2024high}
M. Qin, Y. Liu, Y. Xu, X. Zhao, Y. Liu, and H. Wang, ``High-fidelity 3d head avatars reconstruction through spatially-varying expression conditioned neural radiance field,'' in \textit{Proceedings of the AAAI Conference on Artificial Intelligence}, vol. 38, no. 5, pp. 4569--4577, 2024.

\bibitem{xie2024g}
S. Xie, S. Zhou, K. Sakurada, R. Ishikawa, M. Onishi, and T. Oishi, ``G 2 f R: Frequency Regularization in Grid-Based Feature Encoding Neural Radiance Fields,'' in \textit{European Conference on Computer Vision}, pp. 186--203, 2024.

\bibitem{li2024spectralnerf}
R. Li, J. Liu, G. Liu, S. Zhang, B. Zeng, and S. Liu, ``Spectralnerf: Physically based spectral rendering with neural radiance field,'' in \textit{Proceedings of the AAAI Conference on Artificial Intelligence}, vol. 38, no. 4, pp. 3154--3162, 2024.

\bibitem{bengio2009curriculum}
Y. Bengio, J. Louradour, R. Collobert, and J. Weston, ``Curriculum learning,'' in \textit{Proceedings of the 26th annual international conference on machine learning}, pp. 41--48, 2009.

\bibitem{lu2025lsf}
X. Lu, C. Zhuang, C. Jin, Z. Lu, Y. Wang, W. Liu, and J. Xiao, ``LSF-Animation: Label-Free Speech-Driven Facial Animation via Implicit Feature Representation,'' in \textit{Proceedings of the SIGGRAPH Asia 2025 Conference Papers}, pp. 1--12, 2025.

\bibitem{zhang2023sdrnet}
S. Zhang, F. Song, G. Song, and M. Yang, ``Sdrnet: Shape decoupled regression network for 3d face reconstruction,'' in \textit{ICASSP 2023-2023 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, pp. 1--5, 2023.

\end{thebibliography}
